Anti-Tamper Radio meets Reconfigurable Intelligent Surface for System-Level Tamper Detection

Many computing systems need to be protected against physical attacks using active tamper detection based on sensors. One technical solution is to employ an ATR (Anti-Tamper Radio) approach, analyzing the radio wave propagation effects within a protected device to detect unauthorized physical alterations. However, ATR systems face key challenges in terms of susceptibility to signal manipulation attacks, limited reliability due to environmental noise, and regulatory constraints from wide bandwidth usage. In this work, we propose and experimentally evaluate an ATR system complemented by an RIS to dynamically reconfigure the wireless propagation environment. We show that this approach can enhance resistance against signal manipulation attacks, reduce bandwidth requirements from several~GHz down to as low as 20 MHz, and improve robustness to environmental disturbances such as internal fan movements. Our work demonstrates that RIS integration can strengthen the ATR performance to enhance security, sensitivity, and robustness, recognizing the potential of smart radio environments for ATR-based tamper detection

==> formulas.tex <==





















==> includes_and_commands.tex <==
\usepackage{tikz}

\usepackage{xcolor}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
     T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}


\newcommand{\bcirc}[1]{\tikz[baseline=(myanchor.base)] \node[circle,fill=.,inner sep=1pt] (myanchor) {\color{-.}\bfseries\footnotesize #1};}

\usepackage[mode=buildnew]{standalone}%
\usepackage{tikz}
\usetikzlibrary{patterns}
\usetikzlibrary{positioning,shapes.misc}
\usetikzlibrary{arrows,fit,calc,automata}

\usepackage{svg}

\usepackage[ruled,vlined, linesnumbered]{algorithm2e} %
\usepackage{csquotes}
\usepackage{pgfplots}
\SetKwComment{Comment}{/* }{ */}
\RestyleAlgo{ruled}
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKw{go}{goto}
\usepackage{pifont}
\usepackage{placeins}
\usepackage{multirow}
\usepackage{comment}

\usepackage[nolist]{acronym}
\usepackage{float}


\usepackage{eurosym}
\usepackage{enumitem}

\usepackage[binary-units=true]{siunitx}

\usepackage{caption}
\usepackage{subcaption}
\usepackage{graphicx}

\usepackage{booktabs}

\usepackage{listings}
\usepackage{minted}
\usepackage{multirow}
\usepackage{diagbox}
\usepackage{cancel}

\usepackage{colortbl}
\usepackage{zref-savepos}
\usepackage{pict2e}
\usepackage{wasysym}

\usepackage{array}
\usepackage{hhline}

\usepackage{natbib}
\usepackage{xurl}

\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\newcommand{\fcircle}{\ding{108}}%
\newcommand{\ftriangle}{\ding{115}}%
\newcommand{\fsquare}{\ding{110}}%
\newcommand{\cross}{\ding{53}}%


\newcommand{\philipp}[1]{\todo[color=yellow, textcolor=red]{#1}}
\newcommand{\paul}[1]{\todo[color=lime, textcolor=red]{#1}}
\newcommand{\vm}[1]{\todo[color=olive, textcolor=red]{#1}}
\newcommand{\important}[1]{\todo[color=red, textcolor=red]{#1}}

\newsavebox{\largestimage}

\newcounter{NoTableEntry}
\renewcommand*{\theNoTableEntry}{NTE-\the\value{NoTableEntry}}

\newlength{\plotwidth}
\setlength{\plotwidth}{0.85\columnwidth}


\makeatletter
\newcommand*{\notableentry}{%
  \kern-\tabcolsep
  \stepcounter{NoTableEntry}%
  \vadjust pre{\zsavepos{\theNoTableEntry t}}%
  \vadjust{\zsavepos{\theNoTableEntry b}}%
  \zsavepos{\theNoTableEntry l}%
  \raisebox{%
    \dimexpr\zposy{\theNoTableEntry b}sp
    -\zposy{\theNoTableEntry l}sp\relax
  }[0pt][0pt]{%
    \color{black}%
    \setlength{\unitlength}{1pt}%
    \edef\w{%
      \strip@pt\dimexpr\zposx{\theNoTableEntry r}sp%
      -\zposx{\theNoTableEntry l}sp\relax
    }%
    \edef\h{%
      \strip@pt\dimexpr\zposy{\theNoTableEntry t}sp%
      -\zposy{\theNoTableEntry b}sp\relax
    }%
    \ifdim\w pt=0pt %
    \else
      \begin{picture}(0,0)%
        \edef\x{%
          \noexpand\put(0,0){\noexpand\line(\w,\h){\w}}%
          \noexpand\put(0,\h){\noexpand\line(\w,-\h){\w}}%
        }\x
      \end{picture}%
    \fi
  }%
  \hspace{0pt plus 1filll}%
  \zsavepos{\theNoTableEntry r}%
  \kern-\tabcolsep
}   

